The Law of Knowledge Overshadowing: Towards Understanding, Predicting, and Preventing LLM Hallucination

Hallucination is a persistent challenge in large language models (LLMs), where even with rigorous quality control, models often generate distorted facts. This paradox, in which error generation continues despite high-quality training data, calls for a deeper understanding of the underlying LLM mechanisms. To address it, we propose a novel concept: knowledge overshadowing, where model's dominant knowledge can obscure less prominent knowledge during text generation, causing the model to fabricate inaccurate details. Building on this idea, we introduce a novel framework to quantify factual hallucinations by modeling knowledge overshadowing. Central to our approach is the log-linear law, which predicts that the rate of factual hallucination increases linearly with the logarithmic scale of (1) Knowledge Popularity, (2) Knowledge Length, and (3) Model Size. The law provides a means to preemptively quantify hallucinations, offering foresight into their occurrence even before model training or inference. Built on overshadowing effect, we propose a new decoding strategy CoDa, to mitigate hallucinations, which notably enhance model factuality on Overshadow (27.9%), MemoTrap (13.1%) and NQ-Swap (18.3%). Our findings not only deepen understandings of the underlying mechanisms behind hallucinations but also provide actionable insights for developing more predictable and controllable language models.

==> figures/decay.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[height=0.65in]{figures/plotA.pdf}
    \label{fig:weight}
    \includegraphics[height=0.65in]{figures/plotB.pdf}
    \label{fig:ratio}
    \includegraphics[height=0.65in]{figures/plotC.pdf}
    \label{fig:length}
    \label{fig:generalization-factors}
        \caption{Controllable variants affect hallucination rate (\%) and GSNR (generalization). \textcolor{blue}{put b and c figures in appendix}}
\end{figure}

==> figures/domains.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{pictures/domains.jpg}
    \caption{knowledge overshadowing in deductive logical reasoning, mathematical calculation, and knowledge conflicts. \textcolor{gray}{Grey} refers to the overshadowed tokens. \textcolor{blue}{Blue} refers to the more popular knowledge. \textcolor{orange}{Orange} refers to the hallucinated output.}\label{fig:domains}
\end{figure}

==> figures/generalization_hallucination.tex <==
\begin{figure}[htb]
\centering
\subfloat{\includegraphics[height=1.4in]{pictures/plotA.pdf}%
\label{fig:eliminator1}}
\vspace{-0.8em}
\caption{Gradient-Signal-Noise-Ratio is applied to quantify generalization. As growing weight decay boosts generalization, hallucination caused by knowledge overshadowing steadily grows with generalization.}
\label{fig:eliminator}
\vspace{-0.9em}
\end{figure}

==> figures/length.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[height=0.72in]{figures/plot_pythia.pdf}
    \label{fig:compare1}
    \includegraphics[height=0.72in]{figures/plot_phi.pdf}
    \label{fig:compare2}
    \includegraphics[height=0.72in]{figures/plot_gptj.pdf}
    \label{fig:compare3}
    \includegraphics[height=0.72in]{figures/plot_llama.pdf}
    \label{fig:compare4}
    \label{fig:enter-label}
        \caption{Hallucination rate (\%) with varying prefix lenghts on varying model families. }
\end{figure}

==> sections/experiment.tex <==
\section{Experimental Results}

%In this section, we first compare our method performance with other comparisons. Then we conduct quantitative and qualitative analysis to showcase when and why our method performs well. 


\subsection{Main Results}



We first experiment with our proposed hallucination alarmer to anticipate to-be-produced hallucination by the model on a given input. Then we compare our hallucination eliminator SCD with other comparisons.




\paragraph{Performance of Hallucination Alarmer. } 
\textit{Our hallucination alarmer exploiting knowledge overshadowing as the hallucination signal significantly outperforms the baseline on all three datasets.} 
Our hallucination alarmer successfully predicts 25.8\%, 24.7\%, and 47.0\% hallucinated output on MemoTrap, NQ-Swap, and Overshadow on average before full generation, mitigating the research gap of not only evaluating whether a language model will hallucinate but also anticipating the hallucination output with notable performance.


\paragraph{Performance of Hallucination Eliminator (SCD).}
\textit{Our method notably enhances the greedy decoding baseline performance by 27.9\%, 13.1\%, and 18.3\% on Overshadow, MemoTrap, and NQ-Swap benchmarks. }
Our method exhibits robust and superior performance compared with all other methods.

\textit{Baseline methods that elicit deeper reasoning steps of language models compromise their performance on the hallucinations caused by knowledge overshadowing. }
This demonstrates the tenacity of knowledge overshadowing.

\textit{Baseline methods that encourage self-consistency show unstable or even degraded performance on knowledge overshadowing.} The reasons may lie in that enhanced consistency may reinforce over-alignment on pre-trained bias brought by popular knowledge.


\subsection{Quantitative Analysis}
As shown in Figure~\ref{fig:quantitative_analysis}, the relative knowledge popularity level (r-KP) and the relative knowledge representation length (r-KL) can greatly influence knowledge overshadowing.
Hence we conduct quantitative analysis on model results of the synthetic dataset with controlled r-KL and r-KP to investigate how our hallucination eliminator SCD performs by varying r-KL and r-KP. 

\input{figures/eliminator}


As shown above, as the r-KL and r-KP increase, consistent with our previous findings, hallucination caused by knowledge overshadowing becomes more tenacious, namely, the more popular knowledge is generalized, the harder to excavate valuable information from the over-suppressed knowledge representations.


\subsection{Case study}

Here we showcase how our hallucination alarmer and eliminator (SCD) work with illustrations.

The popular knowledge introduced in the pre-training stage is the well-known quote ``Actions speak louder than words''. 
The contextual knowledge instructing the model to output ``Actions speak louder than thoughts'' is less popular and consequently overshadowed by the more popular original quote.
When the word ``thoughts'' representing less popular contextual knowledge is masked, the new input represents the more popular knowledge only.
Thus we can downweight the more popular knowledge (``Actions speak louder than'' associated with ``words'') by self-contrastive decoding. 
Specifically, the word ``thoughts'' encodes the overshadowed contextual knowledge in this case. 
After the contrastive decoding to downweight popular association between ``Actions speak louder than'' and ``words'', the correct output ``thoughts'' emerges.

==> sections/setup.tex <==
\section{Experimental Setup}
In this section, we introduce datasets and baselines for the experimental setup.



% \subsection{Datasets}
% We experiment on two public datasets that explore hallucinations caused by conflicting knowledge and our Overshadowing dataset.

% Memotrap in appendix

% NQ-SWAP in appendix

% \paragraph{Overshadow. }
% As elaborated in \S~\ref{sec:formulation} (more details in~\ref{ssec: overshadowing_dataset}), our Overshadowing dataset contains more popular and less popular knowledge sets with varying relative knowledge popularity levels and relative knowledge representation levels, which will be utilized for further quantitative analysis.





% \subsection{Comparison Baselines}


% \paragraph{Hallucination Alarmer Comparisons. }
% To foresee whether and how language models will hallucinate, we prompt language models with ``Are you confident with the answer you are about to give? If not, what is the answer you are about to give?'' to judge whether they will hallucinate.
% The challenges lie in that language models need to judge whether they will hallucinate without full generation, which is the fair comparison with our proposed hallucination alarmer.


% \paragraph{Hallucination Elimination  Comparisons.}
% We compare our Self-Contrastive Decoding (SCD) method with baselines as follows:

% \textit{Greedy decoding} is the baseline of outputting tokens with optimal probability.
% We prompt language models to answer each question by \textit{Chain-of-Thought (Cot)} to involve deeper reasoning~\cite{wei2022chain}.
% \citet{madaan2024self} proposed \textit{Self-Reflection (SR)} to combine multiple sampled responses into a single input and then prompt the model to analyze the factual information from these sampled responses to generate a new, more accurate response.
% \citet{chen2023universal} proposes \textit{USC} to instruct LLMs to select the most consistent responses from their sampled responses.
% \citet{chuang2023dola} eliminated hallucinations by \textit{Dola} to identifying hallucinations in contrastive model layers. 


% \paragraph{Implementationa and Metric. }
% For the hallucination alarmer evaluation, we adopt accuracy as the metric. If we not only foresee the model will hallucinate but also predict the specific hallucinated output, the success prediction counts.
% For the hallucination elimination evaluation, we use the Exact Match (EM) metric following previous practices~\cite{longpre-etal-2021-entity}. Implementation details are elaborated in~\ref{ssec:implementation}.



==> sections/theory.tex <==
\section{Knowledge Overshadowing as a Case of Over-Generalization }
\label{sec:theory}
Why does knowledge overshadowing happen at all? We first measure the generalization ability of the model and show that the hallucination rate is closely related to model generalization, showing that knowledge overshadowing is a case of over-generalization. Then we analyze the generalization bound of the model and show its connections with the imbalance ratio and condition length. 


\paragraph{Generalization positively correlates with hallucination.}
%The generalization error bound theoretically explains that generalization of popular patterns lead to hallucinations. Furthermore, we empirically explore the consistency between generalization and hallucination.
We quantify model generalization with Gradient
signal-to-noise ratio (GSNR)~\cite{liu2020understanding}. 
We utilize GSNR to measure the similarity of gradients among different training samples. A large GSNR indicates higher agreement of the optimizing direction on gradients in training time, then parameters are prone to be ``associated with a pattern'', which leads to the better generalization. From Figure \ref{fig:generalization-factors}, we can observe that the hallucination rate correlates well with GSNR over different imbalance ratios and condition lengths. 

%We quantitatively analyze how imbalance ratio, condition length will affect generalization and hallucination.
Weight decay is the well-known regularization for neural networks to enhance model generalization~\cite{wei2019data}, thus we experiment with varying weight decay to boost generalization and observe the resulting hallucination rate. 
The results show that the hallucination rate increases consistently with generalization, and larger weight decay, larger imbalance ratio, and larger condition length all lead to higher generalization and hallucination rate.

\input{figures/decay}

\paragraph{Generalization error bound of auto-regressive language modeling.}
% \pengfei{I think there are a few places for improvements on clarity}
% \pengfei{1. $\boldsymbol{x_{k+1}}$ should have a superscript $i$ where $1\le i \le M$, meaning dominating sequences have varying infixes. }
In the following analysis, we simplify the problem by assuming that the infix condition $B$ is only one token long, so the prefix condition $A$ can be written as  ${x}_1, \dots, {x}_k$, and the infix condition $B$ as ${x}_{k+1}$ so that the relative length would be $k$.
% refers to the infix condition $B$. Then $y$ and $\tilde{y}$ are continuations $C$ conditioning on $A,B$.
Following our experiment setting in \autoref{sec:syn_exp}, we assume that the dataset $\mathbf{D} \sim \mathcal{D}$ is comprised of multiple imbalanced groups. 
Each imbalanced group ${Q}$ includes a subset $Q_M$ of size $M$ with samples $s = ({x}_1, \dots, {x}_k, {x}_{k+1}, y)$, and subset $Q_N$ of size $N$  with samples $\tilde{s} = ({x}_1, \dots, {x}_k, \tilde{{x}}_{k+1}, \tilde{y})$. 
All tokens 
%${x}_1, \dots,{x}_k,{x}_{k+1}, \tilde{{x}}_{k+1}, y, \tilde{y}$ 
are from the vocabulary $\mathcal{V}=\{1, 2, ..., V\}$.
% ~\cite{thrampoulidis2024implicit, vaswani2017attention}. 


% To simplify the question, we formulate $s$ with length of prefix $X$ as $k$, and the length of infix $B$ as one, then the $k/1=$length($A$)/length($B$) represents the relative length of A:B.
% Normally $y$ indicates multi-step next token prediction (NTP). We formulate the sub-question where $y$ includes one token.
%With the imbalance ratio $r=M/N>1$, the more popular prefix condition ${x}_1,\dots, {x}_k$ tends to overshadow the less popular infix condition $\tilde{{x}}_{k+1}$, thus generating the wrong continuation $y$, defined as amalgamated hallucination, whose final output is ${x}_1, \dots, {x}_k, \tilde{{x}}_{k+1}, y$, deviating from the factual dataset. We assume this hallucination is a case of over-generalization of the frequently seen pattern ${x}_1, \dots, {x}_k, {x}_{k+1}, y$ by language model. Thus we explore the generalizability of the popular samples $s$. 
The next token prediction (NTP) loss for $s$ based on auto-regressive modeling is:
\begin{small}
\begin{equation}
\mathcal{L}_\mathrm{NTP} = \hat{\mathbb{E}}_{{x} \sim Q_M} \left[ \sum_{{x} \in [K+1]} -\log \left( p(y | {x}_1, \dots, {x}_k, {x}_{k+1}) \right) \right]
\end{equation}
\end{small}
% Here $\hat{\mathbb{E}}$ is the expectation over training set $Q$ of sequences $s$ sampled from true distribution.
% Then, the auto-regressive model $\mathcal{M}_{\theta}$ parameterized by $\theta$ is trained on this cross-entropy loss for next token prediction.
% $\mathbf{W_{\theta}}({x}_1, \dots, {x}_k, {x}_{k+1}))$ are the output logits, on which the softmax function $\mathcal{S}$ is applied to output the probability of next token $y$, given the input sequence of $({x}_1, \dots,{x}_k, {x}_{k+1})$:
% \begin{small}
% \begin{equation}
% \begin{aligned}
%     p(y | {x}_1, \dots,{x}_k, {x}_{k+1})) & =\mathcal{M}_{\theta}(y | {x}_1, \dots, {x}_k, {x}_{k+1}))= \mathcal{S}_{y} \left( \mathbf{W_{\theta}}({x}_1, \dots, {x}_k, {x}_{k+1})) \right) \\
%     & = \frac{\exp \left( e_y^\top \mathbf{W_\theta}(x_1, \dots, x_k, x_{k+1}) \right)}{ \sum_{{x}' \in \mathcal{V} } \exp \left( e_{{x}'}^\top \mathbf{W_\theta}(x_1, \dots, x_k, x_{k+1}) \right)}
% \end{aligned}
% \end{equation}
% \end{small}
% Here $e_y$ corresponds to the one-hot vector with the $y$-th dimension being 1.s
% Then the parameters $\mathbf{W_{\theta}}$ will be trained by minimizing the cross-entropy loss $\mathcal{L}_\mathrm{NTP}$ by gradient descending. While our focus here is to explore how training data impacts generalization, thus we assume the following analysis holds the same model $\mathcal{M}_{\theta}$.
% \paragraph{Auto-regressive language modeling loss for next token prediction. }
% Different from traditional one-hot classification, the training objective of text generation on an auto-regressive model is the multi-step cross-entropy minimization over the predicted next token, where each predicted token corresponds to an empirical probability distribution over a finite vocabulary determined by the tokenizer~\cite{thrampoulidis2024implicit, vaswani2017attention}. 
% To simplify the token-by-token prediction, we focus on the smallest unit of the whole sentence generation problem, where we formulate the question as a single-token prediction task given an input context.
% Here, in a training set $\mathcal{D}^{n}$, there are $n$ samples of sequences $s_i = (t_1, t_2, .., t_i)$ of varying lengths $i$, consisting of tokens $t$. All tokens are from a finite vocabulary $\mathcal{V}=\{1,2, ..., V\}$.  
% For each training sample, given an input context sequence of $s_{i-1} = (t_1, t_2, .., t_{i-1})$, the auto-regressive model $\mathcal{M}_{\theta}$ parameterized by $\theta$ is trained to predict the next token $t_i$ of the input context $s_{i-1}$ of length $I$ using the cross-entropy loss:
% \begin{small}
% \begin{equation}
% \mathcal{L}_\mathrm{NTP} = \hat{\mathbb{E}}_{t \sim \mathcal{D}^n} \left[ \sum_{t \in [I]} -\log \left( p(y | x_1 \dots x_k, x_{k+1}) \right) \right]
% \end{equation}
% \end{small}
% Here $\hat{\mathbb{E}}$ is the expectation over training set $\mathcal{D}^n$ of sequences $s_i$ sampled from true distribution. Then, 
% \begin{small}
% \begin{equation}
% \begin{aligned}
%     p(y | x_1, \dots x_k, x_{k+1}) & =\mathcal{M}_{\theta}(t_i \mid t_1, \ldots, t_{i-1})= S_{t_i} \left( \mathcal{W}_{\theta}(t_1, \ldots, t_{i-1}) \right) \\
%     & = \frac{1}{1 + \sum_{t' \in \mathcal{V}, t' \neq t_i} \exp \left( (e_{t'} - e_{t_i})^\top \mathcal{W}_{\theta'}(t_1, \ldots, t_{i-1}) \right)}.
% \end{aligned}
% \end{equation}
% \end{small}
% Here $\mathcal{W}_{\theta}(t_1, \ldots, t_{i-1})$ is the output logits, on which the softmax function $S_{t_i}$ is applied to output the probability of next token $t_i$, given the input context $s_{i-1}=(t_1, .., t_{i-1})$.
% Denoting $s_{i-1}$ as the input $x$, $t_i$ as the output $y$, the training set is comprised of feature-label-like pairs $(x, y)$, Then the cross-entropy loss for next token prediction can be rewritten as:
% \begin{equation}\small
% \mathcal{L}_\mathrm{NTP} = \hat{\mathbb{E}}_{x \sim \mathcal{D}^n} \left[  -\log \left( p(y|x) \right) \right] 
% \end{equation}
% The loss resembles the traditional one-hot classification where $x$ is the input feature, and $y$ is the ground-truth label. Then we can conduct the generalization analysis under classification task setting.

Our optimizing objective 
%for next token prediction by auto-regressive language modeling 
is to learn a function $f: \mathcal{X}\rightarrow\mathbb{R}^{V}$, ($\mathcal{X}$ for input space), to minimize the risk $\mathcal{R}_{y}$ defined on the true distribution using NTP as the surrogate loss:
% \begin{small}
% \begin{equation}
% \mathcal{R}_\mathrm{NTP}(f) := \frac{1}{V} \sum_{y=1}^{V} R_{y}(f) = \frac{1}{V} \sum_{y=1}^{V} \mathbb{E}_{{x}_1, \dots, {x}_k, {x}_{k+1} \sim Q_M} [\mathcal{J}(f({x}_1, \dots, {x}_k, {x}_{k+1}), y)]
% \end{equation}
% \end{small}
% Here $\mathcal{R}_{y}$ is the risk of prediction on $y$, referring to mistakes made by models when making prediction, where $\mathcal{J}: 
% \mathbb{R}^{V}\times\mathcal{V}$ is to evaluate the model performance on the true distribution $\mathcal{D}$, from which the training set $Q_M$ is sampled. Since $\mathcal{J}$ is intractable, we adopt the surrogate loss function $\mathcal{L}: \mathbb{R}^{V}\times\mathcal{V}\rightarrow\mathbb{R}_{+}$, here $\mathcal{L}:=\mathcal{L}_\mathrm{NTP}$. Then the risk calculated on surrogate loss is: 
\begin{small}
\begin{equation}
\mathcal{R}^{\mathcal{L}}_\mathrm{NTP}(f) := \frac{1}{V} \sum_{y=1}^{V} \mathcal{R}^{\mathcal{L}}_y(f) = \frac{1}{V} \sum_{y=1}^{V} \mathbb{E}_{{x}_1, \dots, {x}_k, {x}_{k+1} \sim Q_M} [\mathcal{L}(f({x}_1, \dots, {x}_k, {x}_{k+1}), y)]
\end{equation}
\end{small}
Based on the above NTP optimizing objective formulation, the empirical risk can be formulated as:
\begin{equation}
\widehat{\mathcal{R}}^{\mathcal{L}}_\mathrm{NTP}(f) := \frac{1}{M} \sum_{(\boldsymbol{x},y) \in Q_{M}} \mathcal{L}(f(x_1, ..., x_k, x_{k+1}), y)
\end{equation}
\textbf{Proposition 1} (Generalization bound on Rademacher complexity~\cite{mohri2018foundations}).
Let $\mathcal{G}$ be a family of functions. Then, for any $\delta > 0 $, with probability at least $1 - \delta$ over the draw of an i.i.d. (independent and identically distributed) sample $Q_M$ of size $M$, $ \exists \text{ a constant } C > 0, f(t) \le C \cdot g(t)$~\cite{wang2024unified}, the generalization bound holds for all $g \in \mathcal{G}$:
% Given the loss function $\mathcal{L}: \mathbb{R}^{V}\times\mathcal{V}$, and a function set $\mathcal{F}$, where $f \in \mathcal{F}$, then for any $\delta \in (0, 1)$, with probability larger than $1-\delta$ over the training set $\mathcal{D}_n$, the generalization error bound holds for all $f \in \mathcal{G}$:
\begin{small}
\begin{equation}
\label{eq.initial_bound}
\mathcal{R}^{\mathcal{L}}_y(f) \precsim \widehat{\mathcal{R}}^{\mathcal{L}}_y(f) + 2\widehat{\Re}_{Q_M}(\mathcal{G}) + \sqrt{\frac{\log 1/\delta}{2M}} 
\end{equation}
\end{small}
Here ${\Re}_y(\mathcal{G})$ denotes the empirical Rademacher complexity of the function set $\mathcal{G}$, as a measure of the richness of $\mathcal{G}$. 
% $g \in \mathcal{G}$ is to bound expected values and empirical averages on dataset $Q_M$. 
% The generalization bound is still loose for the NTP since it doesn't reveal how more variants of multiple conditions relate to generalization ability. Thus we bound $\mathcal{G}$ tighter. 
Then we employ \textit{Lipschitz Continuity} to further bound the complexity ${\Re}(\mathcal{G})$~\cite{cao2019learning}.

\textbf{Definition 1}(Lipschitz continuity).
With$\|\cdot\|$ denotes the 2-norm, then the function $\mathcal{L}$ is \textit{Lipschitz continuous} with the constant $\mu$ if for any $f, f' \in \mathcal{F}$, $x \in Q$:
\begin{small}
\begin{equation}
|\mathcal{L}(f, y) - \mathcal{L}(f', y)| \leq \mu \cdot \|f(x) - f'(x)\|
\end{equation}
\end{small}
If the NTP loss function $\mathcal{L}_\mathrm{NTP}(f)$ is \textit{Lipschitz continuous} with constant $\mu$, then $\Re_{Q_M}(\mathcal{G})$ could be:
\begin{equation}
\label{eq.bound_rade}
\hat{{\Re}}_{\mathbf{Q_M}}(\mathcal{G}) \le \mu \cdot \hat{{\Re}}_{\mathcal{Q_M}}(\mathcal{F}).
    \end{equation}
%\paragraph{Length-dependency for multiple conditions. }
We derive that the next-token-prediction loss $\mathcal{L}_\mathrm{NTP}$ is \textit{Lipschitz continous} with the constant $\mu=\sqrt{1 + \left( \sum_{y' \neq y} h^{-1}(k) \right)^2} \left[ 1 - \mathrm{softmax}\left( \boldsymbol{s}_{y} \right) \right]$ (See details in \S~\ref{appendix:length_dependency}), by substituting $\mu$ to Eq.(\ref{eq.initial_bound}) and Eq.(\ref{eq.bound_rade}), we derive the more fine-grained generalization bound for NTP with multiple conditions:
\begin{small}
\begin{equation}
\label{eq.final_bound}
\mathcal{R}^{\mathcal{L}}_y(f) \precsim \widehat{\mathcal{R}}^{\mathcal{L}}_y(f) + 2\widehat{\Re}_{Q_M}(\mathcal{F})\sqrt{1 + \left( \sum_{y' \neq y} h^{-1}(k) \right)^2} \left[ 1 - \mathrm{softmax}\left( \boldsymbol{s}_{y} \right) \right] + \sqrt{\frac{\log 1/\delta}{2M}} 
\end{equation}
\end{small}
Here the generalization bound contains two coefficients $M$ and $h(k)$. $M$\footnote{Here we fix the number of suppressed samples to N for simplified generalization analysis. Then M indicates to what extent the dominant condition overshadows suppressed condition.} refers to number of dominant samples of $s_{k+2} = ({x}_1, \dots, {x}_k, {x}_{k+1}, y), s_{k+2} \in Q_{M}$, $h(k)$. $h(k)$ is the value positively correlated with the length of the dominant prefix. Then, the longer length of dominant prefix $({x}_1, \dots, {x}_k)$ and higher dominant ratio lead to lower generalization bound, in other words, better generalization.
The bound provides theoretical insights that hallucination is highly relevant to generalization, 
echoing the experimental results (Table~\ref{tab:nl_results}, Table~\ref{tab:syn_results}, Figure~\ref{fig:generalization-factors}) that over-generalization of dominant patterns overshadow other patterns, leading to amalgamated hallucinations.

% over-generalization of dominant patterns observed in previous experiments (Table~\ref{tab:nl_results}, Table~\ref{tab:syn_results}, Figure~\ref{fig:generalization-factors}). 



==> tables/GPT-hallucination.tex <==
\begin{table}[htb]
\linespread{1.5}
\tabcolsep=0.036cm
\fontsize{7.8pt}{8pt}\selectfont
\caption{A wide range of hallucinations made by GPT-3.5 series of models that can be attributed to knowledge overshadowing.}
\begin{tabular}
{p{2.3cm}@{\hskip 0.2cm}p{4.0cm}@{\hskip 0.2cm}p{7cm}}
\noalign{{\color{black}\hrule height 1pt}}
Overshadowing & Input Prompt & Hallucinated Answer from LLMs  \\ \hline
\textcolor{magenta}{Not won the Nobel prize} \textbf{Overshadowed} \textcolor{cyan}{Nomination} & List some authors that were nominated but did not win the Nobel prize. & 1. Leo Tolstoy 2. James Joyce \sout{\textcolor{magenta}{3. Mark Twain}} 4. Virginia Woolf 5. Jorge Luis Borges \sout{\textcolor{magenta}{6. Emily Dickinson 7. George Orwell}} 8. Anton Chekhov 9. Jorge Amado \sout{\textcolor{magenta}{10. Thomas Hardy }}\\
\hline
\textcolor{magenta}{from Korea} \textbf{Overshadowed} \textcolor{cyan}{rock musicians} & Tell me some rock musicians from Korea. & 1. Yoon Do-hyun 2. Lee Seung-hwan 3. Shin Seung-hun 4. Seo Taiji 5. Kim Kyung-ho 6. Moon Hee-joon 7. Kang San-ae 8. Noh Soo-ram 9. Oh Seung-geun \sout{\textcolor{magenta}{10. Heo Young-saeng}} \\
\hline
\textcolor{magenta}{Description for wining the prize} \textbf{Overshadowed} \textcolor{cyan}{Negation} & Who did not receive the 1921 Nobel Prize in Physics "for his services to theoretical physics, and especially for his discovery of the law of the photoelectric effect"? & \sout{\textcolor{magenta}{German physicist Albert Einstein did not receive the 1921 Nobel}} \sout{\textcolor{magenta}{Prize in Physics for his discovery of the law of the photoelectric}} \sout{\textcolor{magenta}{effect.}} In fact, Einstein was awarded the Nobel Prize in Physics in 1921 for his explanation of the photoelectric effect, which was published in a 1905 paper titled "On a Heuristic Point of View Concerning the Production and Transformation of Light." \\
\hline
\textcolor{magenta}{AI scientist} \textbf{Overshadowed} \textcolor{cyan}{Female} & Tell me some outstanding
female AI scientist. & \sout{\textcolor{magenta}{Yoshua Bengio}}: While not female, Yoshua Bengio has significantly contributed to the advancement of AI and deep learning. As one of the "Three Musketeers of Deep Learning" alongside Geoffrey Hinton and Yann LeCun, his work has had a profound impact on the field. \\
\hline
\noalign{{\color{black}\hrule height 1pt}}
\end{tabular}
\label{tab:gpt_hallu_cases}
\end{table}

==> tables/anticipation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\vspace{-2mm}
% \linespread{0.1}
\begin{subtable}{1.0\linewidth}
\tabcolsep=0.21cm
\fontsize{8.1pt}{9pt}\selectfont
\centering
\begin{tabular}{llccc}
\noalign{{\color{black}\hrule height 1pt}}
Dataset & LM & Average rate & \textbf{Detection (F1 \%)} \\
\noalign{{\color{black}\hrule height 0.5pt}}
\multirow{3}{*}{Celebrity} & Mistral-7B & 80.6{\tiny$\pm 0.5$} & {64.1{\tiny$\pm 0.2$}} \\
& Llama-2-7B & 82.7{\tiny$\pm 0.4$} & {73.8{\tiny$\pm 0.5$}} \\
 & Llama-2-13B & 86.1{\tiny$\pm 0.6$} & {67.5{\tiny$\pm 0.3$}} \\
\noalign{{\color{black}\hrule height 1pt}}
\end{tabular}
\caption{Experimental results on Celebrity dataset.}
\vspace{2mm}
\end{subtable}
\begin{subtable}{1.0\linewidth}
\tabcolsep=0.06cm
\fontsize{7.9pt}{9.9pt}\selectfont
\centering
\begin{tabular}{llcccccc}
\noalign{{\color{black}\hrule height 1pt}}
\multirow{2}{*}{Dataset} & \multirow{2}{*}{LM} & \multirow{2}{*}{Average rate} & \multicolumn{4}{c}{Imbalance ratio} \\ \cline{4-7} 
 &  &  & 10:1 & 25:1 & 50:1 & 100:1 \\
 \noalign{{\color{black}\hrule height 0.5pt}}
\multirow{3}{*}{Synthetic} & Llama-2-7B & 81.0{\tiny$\pm 0.3$} & 68.5{\tiny$\pm 0.4$} & 70.6{\tiny$\pm 0.5$} & 73.4{\tiny$\pm 0.7$} & 82.1{\tiny$\pm 0.4$} \\
 & Phi-2-2.8B & 43.2{\tiny$\pm 0.4$} & 64.7{\tiny$\pm 0.2$} & 64.4{\tiny$\pm 0.6$} & 84.3{\tiny$\pm 0.3$} & 81.4{\tiny$\pm 0.5$} \\
 & Pythia-1B & 35.1{\tiny$\pm 0.2$} & 71.2{\tiny$\pm 0.1$} & 65.3{\tiny$\pm 0.1$} & 59.4{\tiny$\pm 0.4$} & 60.6{\tiny$\pm 0.3$} \\ \cdashline{1-7}[1pt/1pt]
\multirow{3}{*}{Time} & Llama-2-7B & 56.4{\tiny$\pm 0.7$} & 55.3{\tiny$\pm 0.5$} & 58.6{\tiny$\pm 0.7$} & 43.9{\tiny$\pm 0.4$} & 59.4{\tiny$\pm 0.6$} \\
 & Phi-2-2.8B & 35.8{\tiny$\pm 0.2$} & 58.6{\tiny$\pm 0.3$} & 50.0{\tiny$\pm 0.1$} & 45.4{\tiny$\pm 0.1$} & 62.9{\tiny$\pm 0.5$} \\
 & Pythia-1B & 23.6{\tiny$\pm 0.5$} & 47.8{\tiny$\pm 0.7$} & 42.1{\tiny$\pm 0.4$} & 56.6{\tiny$\pm 0.3$} & 49.3{\tiny$\pm 0.6$} \\ \cdashline{1-7}[1pt/1pt]
\multirow{3}{*}{Location} & Llama-2-7B & 63.2{\tiny$\pm 0.5$} & 54.7{\tiny$\pm 0.6$} & 60.6{\tiny$\pm 0.4$} & 72.5{\tiny$\pm 0.6$} & 53.0{\tiny$\pm 0.5$} \\
 & Phi-2-2.8B & 49.4{\tiny$\pm 0.3$} & 46.2{\tiny$\pm 0.4$} & 66.7{\tiny$\pm 0.6$} & 57.1{\tiny$\pm 0.1$} & 60.4{\tiny$\pm 0.3$} \\
 & Pythia-1B & 36.5{\tiny$\pm 0.6$} & 45.4{\tiny$\pm 0.2$} & 59.8{\tiny$\pm 0.1$} & 61.4{\tiny$\pm 0.4$} & 52.5{\tiny$\pm 0.2$} \\ \cdashline{1-7}[1pt/1pt]
\multirow{3}{*}{Gender} & Llama-2-7B & 62.4{\tiny$\pm 0.6$} & 49.3{\tiny$\pm 0.3$} & 61.4{\tiny$\pm 0.5$} & 62.3{\tiny$\pm 0.5$} & 65.8{\tiny$\pm 0.1$} \\
 & Phi-2-2.8B & 50.2{\tiny$\pm 0.2$} & 57.1{\tiny$\pm 0.5$} & 68.3{\tiny$\pm 0.3$} & 52.2{\tiny$\pm 0.2$} & 64.0{\tiny$\pm 0.1$} \\
 & Pythia-1B & 45.3{\tiny$\pm 0.1$} & 42.6{\tiny$\pm 0.6$} & 55.7{\tiny$\pm 0.2$} & 63.8{\tiny$\pm 0.5$} & 62.5{\tiny$\pm 0.4$} \\ \noalign{{\color{black}\hrule height 1pt}}
\end{tabular}
\caption{Comparative results on other four datasets}
\end{subtable}
\caption{Hallucination anticipation (F1: \%) before generation by overshadowing detector. \textcolor{blue}{Main results on the open-book datasets (don't know whether dataset includes $K_a$ or $K_b$): 1. Truthful QA 2. knowledge conflict dataset memoTrap 3. entity conflict dataset NQ}}
\label{tab:hallu_foresee}
\end{table}

==> tables/mitigate.tex <==
\begin{table}[htb]
\vspace{-2mm}
\centering
% \linespread{0.5}
\begin{subtable}{1.0\linewidth}
\tabcolsep=0.11cm
\fontsize{8pt}{9pt}\selectfont
\centering
\begin{tabular}{llcccc}
\noalign{{\color{black}\hrule height 1pt}}
Dataset & LM & Ratio & Zero-shot & RE & SCD (Ours) \\ \noalign{{\color{black}\hrule height 0.5pt}}
\multirow{8}{*}{Synthetic} & \multirow{4}{*}{Llama-2-7B} & 10:1 & 56.3 & 60.4 (\textcolor{purple}{+7.3\%$\uparrow$}) & 38.5 (\textcolor{blue}{-31.6\%$\downarrow$}) \\
 &  & 25:1 & 82.0 & 77.5 (\textcolor{black}{-5.5\%$\downarrow$}) & 69.2 (\textcolor{blue}{-15.6\%$\downarrow$}) \\
 &  & 50:1 & 89.5 & 83.2 (-7.0\%$\downarrow$) & 76.4 (\textcolor{blue}{-14.6\%$\downarrow$}) \\
 &  & 100:1 & 96.1 & 94.7 (-1.5\%$\downarrow$) & 82.6 (\textcolor{blue}{-14.0\%$\downarrow$}) \\ \cdashline{2-6}[1pt/1pt] 
 & \multirow{4}{*}{Phi-2-2.8B} & 10:1 & 37.6 & 41.5 (\textcolor{purple}{+10.9\%$\uparrow$}) & 24.8 (\textcolor{blue}{-34.0\%$\downarrow$}) \\
 &  & 25:1 & 40.1 & 41.4 (\textcolor{purple}{+3.2\%$\uparrow$}) & 27.7 (\textcolor{blue}{-30.9\%$\downarrow$}) \\
 &  & 50:1 & 47.2 & 44.9 (\textcolor{black}{-4.9\%$\downarrow$}) & 35.4 (\textcolor{blue}{-25.0\%$\downarrow$}) \\
 &  & 100:1 & 47.8 & 48.9 (\textcolor{purple}{+2.3\%$\uparrow$}) & 40.1 (\textcolor{blue}{-16.1\%$\downarrow$}) \\ \noalign{{\color{black}\hrule height 0.5pt}}
\multirow{8}{*}{Time} & \multirow{4}{*}{Llama-2-7B} & 10:1 & 45.7 & 43.8 (\textcolor{black}{-4.2\%$\downarrow$}) & 32.3 (\textcolor{blue}{-29.3\%$\downarrow$}) \\
 &  & 25:1 & 50.4 & 55.6 (\textcolor{black}{-10.3\%$\downarrow$}) & 31.4 (\textcolor{blue}{-37.7\%$\downarrow$}) \\
 &  & 50:1 & 58.8 & 61.2 (\textcolor{purple}{+0.4\%$\uparrow$}) & 36.6 (\textcolor{blue}{-37.8\%$\downarrow$}) \\
 &  & 100:1 & 70.5 & 64.5 (\textcolor{black}{-8.5\%$\downarrow$}) & 52.4 (\textcolor{blue}{-25.7\%$\downarrow$}) \\ \cdashline{2-6}[1pt/1pt] 
 & \multirow{4}{*}{Phi-2-2.8B} & 10:1 & 23.1 & 21.6 (\textcolor{black}{-6.5\%$\downarrow$}) & 14.0 (\textcolor{blue}{-39.4\%$\downarrow$}) \\
 &  & 25:1 & 37.5 & 40.2 (\textcolor{purple}{+7.2\%$\uparrow$}) & 25.5 (\textcolor{blue}{-30.7\%$\downarrow$}) \\
 &  & 50:1 & 42.8 & 45.7 (\textcolor{purple}{+6.8\%$\uparrow$}) & 29.6 (\textcolor{blue}{-30.8\%$\downarrow$}) \\
 &  & 100:1 & 50.1 & 49.3 (-1.6\%$\downarrow$) & 37.4 (\textcolor{blue}{-25.3\%$\downarrow$}) \\ \noalign{{\color{black}\hrule height 1pt}}
 \end{tabular}
 \caption{Compative results on Synthetic and Time dataset.}
 \end{subtable}
 \begin{subtable}{1.0\linewidth}
 \centering
 \tabcolsep=0.08cm
\fontsize{8pt}{9pt}\selectfont
 \begin{tabular}{lccccc}
 \noalign{{\color{black}\hrule height 1pt}}
LM & Zero-shot & RE & ICL & CoT & SCD (Ours) \\  \noalign{{\color{black}\hrule height 0.5pt}}
 Mistral-7B & 80.6 & 82.7 \textcolor{purple}{\tiny(+2.6\%$\uparrow$)} & 80.9 \textcolor{purple}{\tiny(+0.3\%$\uparrow$)} & 78.5 \textcolor{black}{\tiny(-2.6\%$\downarrow$)} & 65.3 \textcolor{blue}{\tiny(-19.0\%$\downarrow$)} \\
 Llama-2-7B & 82.7 & 83.3 \textcolor{purple}{\tiny(+1.0\%$\uparrow$)} & 
 81.4 \textcolor{black}{\tiny(-1.6\%$\downarrow$)} & 79.2 {\tiny(-4.2\%$\downarrow$)} & 69.0 \textcolor{blue}{\tiny(-16.6\%$\downarrow$)} \\
 Llama-2-13B & 86.1 & 80.8 {\tiny(-6.1\%$\downarrow$)} & 83.6 {\tiny(-2.9\%$\downarrow$)} & 87.1 \tiny\textcolor{purple}{(+1.1\%$\uparrow$)} & 76.4 \textcolor{blue}{\tiny(-11.2\%$\downarrow$)} \\
\noalign{{\color{black}\hrule height 1pt}}
\end{tabular}
\caption{Comparative results on Celebrity dataset.}
\end{subtable}
\caption{Comparison between SCD and others for hallucination mitigation (hallucination rate: \%).}
\label{tab:hallu_mitigation}
\end{table}


==> tables/probing_table.tex <==
\begin{table}[htb]
\linespread{1.5}
\tabcolsep=0.046cm
\fontsize{7.8pt}{8pt}\selectfont
\caption{Pretrained language models exhibit hallucination in the form of knowledge overshadowing. }
\begin{tabular}
{p{3.5cm}@{\hskip 0.5cm}p{4cm}p{4cm}p{2.5cm}}
\noalign{{\color{black}\hrule height 1pt}}
Prompt & GPT3 & OLMo  & Data Imbalance Ratio \\ \hline
Tell me some outstanding \textcolor{orange}{female} AI scientists... 
& \texttt{Feifei Li, Cynthia Breazeal,  \sout{\textcolor{magenta}{Yann LeCun (male)}}, Anca Dragan}
& \texttt{Feifei Li, \sout{\textcolor{cyan}{Emine Saner (journalist)}}, \sout{\textcolor{magenta}{Yann LeCun (male)}}, \sout{\textcolor{magenta}{Yoshua Bengio (male)}}} & Male AI Scientist VS Female AI Scientist:  431:0  \\
\hline
Tell me some outstanding \textcolor{orange}{male} nurses 
& \texttt{\textcolor{magenta}{\sout{Florence Nightingale}, \sout{Lillian Wald}}, Luther Christman, \sout{\textcolor{cyan}{Harold Koenig(psychiatrist)}}}
& \texttt{Drew Elliott, Michael Pettigrew, John Holland, \sout{\textcolor{cyan}{Stephen Reisinger (soccer)}}, \sout{\textcolor{magenta}{Danielle Haddad (female)}}} & 112177:5124 ('nurse' vs. 'male'+'nurse'), no 'female' word because people assume most of nurses are female\\
\hline
% Tell me some outstanding \textcolor{orange}{black} scientists 
% & Neil deGrasse Tyson, Mae Jemison, George Washington Carver, Percy Julian 
% & \sout{\textcolor{magenta}{George Smith (white)}}, \sout{\textcolor{cyan}{Daniel Chee Tsui (asian)}}, \sout{\textcolor{magenta}{Linton Wells II (white)}},  \sout{\textcolor{cyan}{Dorothy J. Hart (actress)}} &  \\
% \hline
Tell me some famous \textcolor{orange}{homosexual} marriages 
& 
\texttt{David Furnish and Elton John, 
Ellen DeGeneres and Portia de Rossi,
George Takei and Brad Altman,
Neil Patrick Harris and David Burtka}
& \texttt{\textcolor{magenta}{\sout{Barack Obama and Michelle} \sout{Obama (heterosextual)}}, Neil Patrick Gaskarth and David Burtka, Ellen DeGeneres and Portia de Rossi} & 15446:4045 ('famous'+'marriage' vs. 'famous'+'homosextual'+'marriage')\\ 
\hline
Who was \textcolor{orange}{not} a theoretical physicist known for the theory of relativity 
& \texttt{Paul Dirac} 
& \texttt{You are referring to \sout{\textcolor{magenta}{Albert Einstein (affirmation)}}} &11365:7265 ('not a'+'einstein' vs. 'einstein')\\ 
\hline 
Who did \textcolor{orange}{not} receive the 1921 Nobel Prize in Physics ``for his services to theoretical physics, and especially for his discovery of the law of the photoelectric effect''?
& \texttt{German physicist \sout{\textcolor{magenta}{Albert Einstein}} did not receive ...} 
& &\\
\noalign{{\color{black}\hrule height 1pt}}
\end{tabular}
\label{tab:probing}
\end{table}
